A hybrid particle volume-of-fluid method for curvature estimation in multiphase flows

We present a particle method for estimating the curvature of interfaces in volume-of-fluid simulations of multiphase flows. The method is well suited for under-resolved interfaces, and it is shown to be more accurate than the parabolic fitting that is employed in such cases. The curvature is computed from the equilibrium positions of particles constrained to circular arcs and attracted to the interface. The proposed particle method is combined with the method of height functions at higher resolutions, and it is shown to outperform the current combinations of height functions and parabolic fitting. The algorithm is conceptually simple and straightforward to implement on new and existing software frameworks for multiphase flow simulations thus enhancing their capabilities in challenging flow problems. We evaluate the proposed hybrid method on a number of two- and three-dimensional benchmark flow problems and illustrate its capabilities on simulations of flows involving bubble coalescence and turbulent multiphase flows.

==> Makefile <==
DOCNAME = main
LATEXMK = latexmk
#LATEXMK = -pdf -pdflatex="pdflatex -shell-escape"

RM = rm -vf
T = ../tool

all: doc
doc: pdf
pdf: $(DOCNAME).pdf

$(DOCNAME).pdf:
	$(LATEXMK) -pdf $(DOCNAME).tex || $(RM) $@

mostlyclean:
	$(LATEXMK) -silent -c -f
	$(RM) *.bbl *-blx.bib

clean: mostlyclean
	$(LATEXMK) -silent -C -f
	$(RM) *.run.xml *.synctex.gz
	$(RM) *.d

merge: merge.tex
merge.tex:
	$T/merge $(DOCNAME).tex > .tmp.tex && cp .tmp.tex merge.tex

split:
	mkdir -p split && \
	cd split && ../$T/split ../merge.tex > $(DOCNAME).tex

lint:
	chktex -f '%f:%l: %m\
' $(DOCNAME).tex

fig: list/fig
list/fig: all
	@echo update $@
	@awk -v RS='[<>]' '  \
/^use/ { gsub(/^\.\.\//, "", $$2); \
         print $$2           \
}' $(DOCNAME).log | sort > $@

OLDIR = overleafloc

overleaf:; $T/$(OLDIR)

zip:
	git archive --format=zip -o main.zip HEAD

zipbbl:
	git rev-parse --short HEAD > rev
	zip -r mainbbl.zip fig main.tex main.bbl main.bib Makefile rev
	rm -f rev

commit:
	git commit -m "update from revision `cat rev`"

PUB = pub

convert_eps:
	[ "$$(basename $$(pwd))" = "$(OLDIR)" ]
	../$T/convert_eps fig $(PUB)/fig -y

copy_pdf:
	[ "$$(basename $$(pwd))" = "$(OLDIR)" ]
	find fig/* -name "*.pdf" -exec cp -v --parents {} $(PUB)  \;

convert_tif:
	[ "$$(basename $$(pwd))" = "$(OLDIR)" ]
	../$T/convert_tif fig $(PUB)/fig -y

replace_ext:
	[ "$$(basename $$(pwd))" = "$(OLDIR)" ]
	cat main.tex \
		| ../$T/replace_ext jpg tif \
		| ../$T/replace_ext png tif \
		| sed s@fig/@fig/@g \
		> $(PUB)/main.tex

pub:
	mkdir -p $(PUB)
	cp main.bib Makefile $(PUB)/
	make replace_ext
	make copy_pdf
	make convert_tif

.PHONY: all clean doc fig lint merge mostlyclean overleaf pdf split zip $(DOCNAME).pdf commit
.PHONY: convert_eps convert_tif replace_ext pub

.SUFFIXES: .pdf .tex


